Benchmarking Differentially Private Synthetic Data Generation Algorithms

This work presents a systematic benchmark of differentially private synthetic data generation algorithms that can generate tabular data. Utility of the synthetic data is evaluated by measuring whether the synthetic data preserve the distribution of individual and pairs of attributes, pairwise correlation as well as on the accuracy of an ML classification model. In a comprehensive empirical evaluation we identify the top performing algorithms and those that consistently fail to beat baseline approaches.

==> app.tex <==

\eat{
\subsection{Quantitative Overview}

\textbf{Optimal Mechanisms} Figure \ref{fig:optimal} shows the rate of a mechanism being the optimal across different metrics, epsilons and datasets. The figure is stratified by four metric categories. From figure, it is not surprising that "Independent+" wins 39\% time for individual distribution similarity since it uses most of the privacy budget to evaluate the distribution for each single attribute. Notice that "MST+" wins 57\% time for the same category. Although in theory "Independent+" should always to be the optimal in this category, we only repeat running the mechanisms 5 times so the sampling error could affect the results.

The optimal rate in the pairwise distribution similarity category again shows "MST+" is the dominant mechanism. Notice that metrics in this category measures the distribution similarity from all pairs of attributes and most pairs of attributes are close to being independent, so "Independent+" can still achieve a non-trivial optimal rate as 19\%. 

The optimal rate in the pairwise correlation similarity category again shows "MST+" is the dominant mechanism. The metrics in this category focus more on capturing the correlation levels instead of concrete distributions, so "Independent+" has a low chance as 2\% to be the optimal. Notice that all of "MST+", "MWEM-PGM+", "PrivBayse" and "Kamino+" have optimal rate more than 10\% in this category. The total sum of optimal rates could be above 100\% due some nulls.

Finally, the optimal rate in the classification category again shows "MST+" is the dominant mechanism. Notice that all of "MST+", "MWEM-PGM+", "PrivBayse" and "Kamino+" have optimal rate more than 8\% in this category. 

\textbf{Average Ranking} Figure \ref{fig:ranking} shows the average ranking of a mechanism across different metrics, epsilons and datasets. The figure is stratified by four metric categories. Unlike the optimal rate figure, this figure gives a more smooth comparison between the mechanisms. 

In terms of the pairwise correlation similarity, most mechanisms have similar average rankings that is between 6 and 7, except that "MST+", "MWEM-PGM+" and "PrivBayes" have higher rankings and "PATEGAN" has lower rankings. 

In terms of the classification accuracy, only mechanisms "MST+", "MWEM-PGM+", "PrivBayes", "Kamino+", "FEM+" and "RAP+" have average rankings higher than the one of "Independent+". Notice that a classifier that is trained on a dataset sampled from a independent model should be close to a majority classifier, so "Independent+" could be viewed as a baseline in this category.

\textbf{Beating Independent+} Figure \ref{fig:beat} shows the rate of a mechanism beating "Independent+" across different metrics, epsilons and datasets. The figure is stratified by four metric categories. "Independent+" could be viewed as a baseline for two categories: pairwise correlation similarity and classification accuracy. From this figure, we found that "PATECTGAN", "DPCTGAN", "RonGauss", "DPGAN" and "PATEGAN" are mechanisms such that one of the "Independent+"-beating rate is below 50\% from these two categories.
}



%\eat{
\begin{table}
\centering
\begin{tabular}{|p{2cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|}
\hline
  \textbf{column} & \multicolumn{3}{l|}{capital-gain} & \multicolumn{3}{l|}{numerical columns}  \\ \hline
  \bm{$\epsilon$}   & 0.1 & 1.0 & 10.0               & 0.1 & 1.0 & 10.0              \\ \hline
 \textbf{equal-width}  & 0.54 & 0.54 & 0.54 & 0.78 & 0.78 & 0.78  \\ \hline
 \textbf{PrivTree} & 0.97 & 0.99 & 0.99 & 0.90 & 0.97 & 0.96 \\ \hline  
\end{tabular}
\caption{L1 score of "Independent" (with 100 equal-width bins) and "Independent+" (with PrivTree bins) for numerical columns from "adult". The scores for "numerical columns" in the table is the average of all the scores of numerical columns.}
\label{tbl:privtree}
\end{table}
%}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{"figures/Baseline.png"}
    \caption{Raw score of "CorAcc" and "XGBoost" for some selected datasets at $\epsilon=10$. A blue (brown) color indicates it is lower (higher) than the baseline. }
    \label{fig:baseline}
\end{figure}


\subsection{Mechanisms}

We collected open source implementations for each mechanism we considered.  Each mechanism required writing some glue code to run on the datasets used in this benchmark.  The required modifications differed by mechanism, with some mechanisms requiring more work than others.  

For example, several mechanisms expect discrete data as input, while other mechanisms expect continuous data as input.  However, most of the datasets in our benchmark contain mixed column types, which are not natively supported by many of the mechanism implementations we collected.  To deal with this, we wrote general-purpose pre-processing functions that can convert categorical columns to numerical columns (via one-hot encoding) and can convert numerical columns to categorical columns (via discretization). This enabled the mechanisms to run on all of the datasets we considered and we name this step as algorithm repair \cite{DBLP:conf/sigmod/HayMMCZ16}.  

Some mechanisms required more work beyond this.  For example, Kamino provided no interface for setting the privacy parameters $(\epsilon, \delta)$, in favor of reporting the achieved privacy post-hoc.  Thus, to run it for a given privacy budget required deriving hyper-parameters that achieved the desired privacy level.  

Several mechanisms have a large number of hyper-parameters.  In all experiments, we used default hyper-parameters settings found in the open source implementation.  With proper tuning, the performance of mechanisms with many hyper-parameters could be improved.  However, conducting this hyper-parameters search privately can come at a high computational cost and a modest privacy cost. 

Some mechanisms, like MWEM+PGM, FEM, and RAP have the added flexibility to specify a \emph{workload}, or the desired set of queries to preserve.  For these mechanisms, we consistently gave these mechanisms a default workload using the following rules:

\begin{enumerate}
    \item If a label column not present, the workload is all 2-way marginals. 
    \item If a label column is present, the workload is all 2- and 3-way marginals involving the label.  
\end{enumerate}

This workload captures the fact that for labeled datasets, we generally want to preserve the conditional distribution of the label given other attributes to do well on machine learning tasks.  

Finally, some mechanisms satisfy bounded-DP (change one record), while others satisfy unbounded-DP (add/remove one record).  Our treatment of this case is consistent with the evaluation used in the NIST synthetic data competition: both are acceptable, and will be run using the same $\epsilon$ values, even though they have slightly different meanings.  This design choice generally favors mechanisms that satisfy unbounded-DP, since they can generally add $2\times$ less noise.  

\subsection{System}
The benchmark system we designed extends an already establish benchmark system for synthetic data called SDGym.  We utilize SDGyms evaluation environment to run experiments on many datasets and evaluate them using several utility metrics.  While SDGym was originally designed for non-private synthetic data generation algorithms, we are primarily interested in evaluating synthetic data generation mechanisms that satisfy the rigorous notion of $(\epsilon, \delta)$-differential privacy. In this benchmark, we fix $\delta$ as $10^{-7}$ and vary $\epsilon$ from $\{0.1, 1.0, 10.0\}$.

\subsection{Execution environment}

Experimetns were conducted using AWS Parallel Cluster.  Our comptue cluster consisted of two types of nodes: c5.xlarge instances (4 vCPUs and 4GB RAM) and m4.xlarge (2 vCPUs and 16 GB RAM) instances.  We ran most mechanisms on c5.xlarge instances, with the exception of Kamino and RAP, which required more memory.  Each mechanism was run for a maximum of 4 hours on each dataset, epsilon, and trial.  While some mechanisms may have completed given more time, this time limit is consistent with the time limit imposed in the NIST 2020 synthetic data competition.  Furthermore, as we will show experimentally later, mechanisms that didn't run under the four hour time limit on some datasets, generally weren't competitive on the other datasets anyway.



Table \ref{tab:exclusion} is the algorithms that we considered but not included in this benchmark or we tested but there were some issues. %\yt{We might need to have a section for discussing about these algorithms.}

\begin{table}[h]
    \centering
    \begin{tabular}{|p{2.5cm}|p{3cm}|p{2.5cm}|}
    \hline
        Algorithm & Published In & Violated Inclusion Criteria \\ \hline
        PrivateIMLE  \tablefootnote{The original paper is not differentially private. BorealisAI adapted the original algorithm and claimed it follows differential privacy.} & CoRR \cite{DBLP:journals/corr/abs-1809-09087} & Selected Field  \\ \hline
        DPSynthesizer / DPCopula  & PVLDB \cite{DBLP:journals/pvldb/LiXZJ14} & Open Source  \\ \hline
        DPSyn & CoRR \cite{DBLP:journals/corr/abs-2106-12949} & Open Source \\ \hline
        PrivSyn & CoRR \cite{DBLP:journals/corr/abs-2012-15128} & Open Source  \\ \hline
        PMWPub & ICML \cite{DBLP:conf/icml/LiuV0UW21} & No Extra Data  \\ \hline
        PEP / GEM / GEMPUB  & CoRR \cite{DBLP:journals/corr/abs-2106-07153} & Selected Field  \\ \hline
        pMSE & PSD \cite{DBLP:conf/psd/SnokeS18} & Open Source  \\ \hline
        DP-MERF \tablefootnote{It supports tabular data and is implemented by ParkLabML} & AISTATS \cite{DBLP:conf/aistats/HarderAP21} & Selected Field   \\ \hline
        DP-CGAN & CVPR(W) \cite{DBLP:conf/cvpr/Torkzadehmahani19} & Selected Field  \\ \hline
        GS-WGAN & NeurIPS \cite{neurips20chen} & Tabular Data  \\ \hline
        
    \end{tabular}
    \caption{Algorithms considered but not included or found some issues.}
    \label{tab:exclusion}
\end{table}

\eat{
\begin{table*}[h!]
    \centering
    {\small 
    \begin{tabular}{|p{2.8cm}|p{1.5cm}|p{1.5cm}|p{2.8cm}|p{3cm}|p{3.5cm}|}
    \hline
        \textbf{Algorithm} & 
        \textbf{Publish} & 
        \textbf{Imple-mentation} & 
        \textbf{Algorithm \newline Repair} &
        \textbf{Data Model} &
        \textbf{Data Interaction}
        \\ \hline
        \algo{MST} \cite{DBLP:journals/corr/abs-2108-04978} & JPC & McKenna & PrivTree binning & Markov random field & k-way marginals \\ \hline 
        \algo{MWEM-PGM} \cite{mckenna2019graphical} & ICML  &  McKenna & PrivTree binning, selected workload & Markov random field & k-way marginals / workload queries \\ \hline
        \algo{PrivBayes} \cite{DBLP:conf/sigmod/ZhangCPSX14, zhang2017privbayes} & SIGMOD   & SDGym & N/A & Bayesian network & k-way marginals \\ \hline
        \algo{DPGAN} \cite{DBLP:journals/corr/abs-1802-06739} & CoRR  & SmartNoise & one-hot encoding & GAN & sub-sampled gradients \\ \hline
        \algo{DPCTGAN} \cite{rosenblatt2020differentially} & CoRR  & SmartNoise & N/A & CTGAN & sub-sampled gradients \\ \hline
        \algo{PATEGAN} \cite{DBLP:conf/iclr/JordonYS19a} & ICLR  & SmartNoise & one-hot encoding & GAN & sub-sampled gradients  \\ \hline
        \algo{PATECTGAN} \cite{rosenblatt2020differentially} & ICLR  & SmartNoise & N/A & CTGAN & sub-sampled gradients \\ \hline
        \algo{Kamino} \cite{DBLP:journals/pvldb/GeMHI21} & PVLDB  & Ge  & PrivTree binning, parameter setting & AimNet & projected  sub-sample \ry{not familiar with Kamino enough.  What is being projected?} \yt{Each step in the big loop of Kamino will try using the first k-columns to predict the (k+1)-th column, so I say it is projected on the first (k+1) columns to learn a new model.} \\ \hline
        \algo{FEM} \cite{DBLP:conf/icml/VietriTBSW20} & ICML  & Vietri & PrivTree binning, selected workload & N/A & workload queries \\ \hline
        \algo{RAP} \cite{DBLP:conf/icml/AydoreBKKM0S21} & ICML  & Amazon &  PrivTree binning, selected workload & Relaxed tabular & workload queries \\ \hline
        \algo{RON-GAUSS} \cite{DBLP:journals/popets/ChanyaswadLM19} & PETS  & BorealisAI &  one-hot encoding & Gaussian generative model & RON projection \\ \hline
        \algo{GretelRNN} \cite{gretel} & N/A & Gretel & N/A & RNN & sub-sampled gradients \\ \hline

    \end{tabular}
    \caption{Summary of mechanisms included by the inclusion criteria.}
    \label{app:tab:inclusion}
    }
\end{table*}
}

==> benchmark.tex <==
\section{Benchmark Setup}

The benchmark system we designed extends an already establish benchmark system for synthetic data called SDGym.  We utilize SDGyms evaluation environment to run experiments on many datasets and evaluate them using several utility metrics.  While SDGym was originally designed for non-private synthetic data generation algorithms, we are primarily interested in evaluating synthetic data generation mechanisms that satisfy the rigorous notion of $(\epsilon, \delta)$-differential privacy. 

\subsection{Datasets}

In this benchmark we consider a collection of 11 datasets.  Each dataset has different sizes and characteristics.  Some contain numerical data, some contain categorical data, and others contain both.  Some datasets contain a 'label' column for classification while others do not.  

Many datasets listed here are available directly in SDGym's benchmark suite, while others were added as part of our extension.  

\begin{table}[H]
    \centering
    \begin{tabular}{c|cccc}
    Name & Records & Categorical Columns & Numerical Columns & Label \\\hline
    Adult & 32561 & 9 & 6 & Yes \\
    Asia & 20000 & 8 & 0 & No \\
    Census & 299285 & 29 & 12 & Yes \\
    Covtype & 581012 & 1 & 54 & Yes \\
    EchoNASDAQ & 51980 & 3 & 4 & No \\
    Intrusion & 494021 & 4 & 37 & Yes \\
    Adult & 48842 & 9 & 6 & Yes \\
    Bank & 45211 & 13 & 8 & Yes \\
    Car & 1728 & 7 & 0 & Yes \\
    Mushroom & 8124 &  23 & 0 & Yes \\
    Shopping & 12330 & 9 & 10 & Yes \\
    Scooter & 27715 & 0 & 5 & No \\
    \end{tabular}
    \caption{Summary of datasets considered in this benchark study.}
    \label{tab:datasets}
\end{table}

\subsection{Mechanisms}

We collected open source implementations for each mechanism we considered.  Each mechanism required writing some glue code to run on the datasets used in this benchmark.  The required modifications differed by mechanism, with some mechanisms requiring more work than others.  

For example, several mechanisms expect discrete data as input, while other mechanisms expect continuous data as input.  However, most of the datasets in our benchmark contain mixed column types, which are not natively supported by many of the mechanism implementations we collected.  To deal with this, we wrote general-purpose pre-processing functions that can convert categorical columns to numerical columns (via one-hot encoding) and can convert numerical columns to categorical columns (via discretization).  This enabled the mechanisms to run on all of the datasets we considered.  

Some mechanisms required more work beyond this.  For example, Kamino provided no interface for setting the privacy parameters $(\epsilon, \delta)$, in favor of reporting the achieved privacy post-hoc.  Thus, to run it for a given privacy budget required deriving hyper-parameters that achieved the desired privacy level.  

Several mechanisms have a large number of hyper-parameters.  In all experiments, we used default hyper-parameters settings found in the open source implementation.  With proper tuning, the performance of mechanisms with many hyper-parameters could be improved.  However, conducting this hyper-parameters search privately can come at a high computational cost and a modest privacy cost. 

Some mechanisms, like MWEM+PGM, FEM, and RAP have the added flexibility to specify a \emph{workload}, or the desired set of queries to preserve.  For these mechanisms, we consistently gave these mechanisms a default workload using the following rules:

\begin{enumerate}
    \item If a label column not present, the workload is all 2-way marginals. 
    \item If a label column is present, the workload is all 2- and 3-way marginals involving the label.  
\end{enumerate}

This workload captures the fact that for labeled datasets, we generally want to preserve the conditional distribution of the label given other attributes to do well on machine learning tasks.  


Finally, some mechanisms satisfy bounded-DP (change one record), while others satisfy unbounded-DP (add/remove one record).  Our treatment of this case is consistent with the evaluation used in the NIST synthetic data competition: both are acceptable, and will be run using the same $\epsilon$ values, even though they have slightly different meanings.  This design choice generally favors mechanisms that satisfy unbounded-DP, since they can generally add $2\times$ less noise.  

\subsection{Metrics}

To evaluate the quality of the synthetic data, we used several metrics tracked by SDGym, including CSTest, KSTest, DiscreteKLDivergence, ContinuousKLDivergence, LogisticDection, and MLEfficacyMetrics.  This is a representative set of metrics available in SDGym.  While there are others (like SVCDetection), they are comparable to metrics we have considered (in this case, LogisticDetection).  Additionally, we ignore the ``privacy metrics'' tracked by SDGym, as we believe that is not something that should be tracked empirically, but justified mathematically instead.  

\begin{table}[H]
    \centering
    \begin{tabular}{c|p{10cm}}
        \textbf{Metric Name} & \textbf{Description} (from SDGym documentation) \\\hline\hline
        CSTest & This metric uses the Chi-Squared test to compare the distributions of the two categorical columns. It returns the resulting p-value so that a small value indicates that we can reject the null hypothesis (i.e. and suggests that the distributions are different). \\\hline
        KSTest & This function uses the two-sample Kolmogorov–Smirnov test to compare the distributions of the two continuous columns using the empirical CDF. It returns 1 minus the KS Test D statistic, which indicates the maximum distance between the expteced CDF and the observed CDF values. \\\hline
        DiscreteKLDivergence & MultiColumnPairsMetric based on ColumnPairs DiscreteKLDivergence. This computes the KL divergence and afterwards normalizes the value applying 1 / (1 + KLD). \\\hline
        ContinuousKLDivergence & MultiColumnPairsMetric based on ColumnPairs ContinuousKLDivergence. This approximates the KL divergence by binning the continuous values to turn them into categorical values and then computing the relative entropy. Afterwards normalizes the value applying 1 / (1 + KLD). \\\hline
        LogisticDetection & This metric builds a LogisticRegression Classifier that learns to tell the synthetic data apart from the real data, which later on is evaluated using Cross Validation.  The output of the metric is one minus the average ROC AUC score obtained. \\\hline
        MLEfficacyMetric & This fits a [sklearn model] to the synthetic data and then evaluates it making predictions on the real data. \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\subsection{Execution environment}

\ry{Yuchao, please check}
Experimetns were conducted using AWS Parallel Cluster.  Our comptue cluster consisted of two types of nodes: c5.xlarge instances (4 vCPUs and 4GB RAM) and m4.xlarge (2 vCPUs and 16 GB RAM) instances.  We ran most mechanisms on c5.xlarge instances, with the exception of Kamino and RAP, which required more memory.  Each mechanism was run for a maximum of 4 hours on each dataset, epsilon, and trial.  While some mechanisms may have completed given more time, this time limit is consistent with the time limit imposed in the NIST 2020 synthetic data competition.  Furthermore, as we will show experimentally later, mechanisms that didn't run under the four hour time limit on some datasets, generally weren't competitive on the other datasets anyway.  





==> conclusion.tex <==
\section{Conclusion and Future Work}

1) Discretization and embedding are important. Improvement on embedding.

==> cut.tex <==
\subsection{Finding 1: Graphical Models Dominate}

Fixing a setting, which contains a specific metric, dataset and epsilon, we can rank the mechanism according to the average scores. We denote the mechanism with the highest ranking as the optimal mechanism for that setting. If the mechanism didn't run for some specific setting, we give null for its ranking and mark it as non-optimal.

Although there is no single mechanism that is optimal for all the settings, in general graphical-model based mechanisms have a better performance than the alternatives. Figure \ref{fig:optimal} shows the rate of a mechanism being the optimal across different metrics, epsilons and datasets. The figure is stratified by four metric categories. Figure \ref{fig:ranking} shows the average ranking instead. From the optimal-rate figure \ref{fig:optimal}, we found that \algo{MST+} has the highest optimal rate among all the mechanisms. In terms of average ranking from Figure \ref{fig:ranking}, both \algo{MST+} and \algo{MWEM-PGM+} are ranked in average among top-3.


To illustrate the quality of a synthetic dataset, in Figure \ref{fig:qualitative} we plot the pairwise correlations among attributes and a 2-way marginal distribution from the synthetic datasets generated by different mechanisms. We also include the ground truth and a naive algorithm \algo{Independent+} as a reference which assumes all columns are independent and add Laplace noise to each one-way marginal. Specifically, Figure \ref{fig:correlation} illustrates the correlation heatmap of all pairwise categorical attributes for one synthetic data generated by each algorithm given the private data "Adult" and $\epsilon=10.0$. The color map is discrete and corresponding to four correlation levels. The number in the attribute name indicating the domain size.\mh{this seems busy to me, and redundant; should attributes be ordered in some way? e.g., by domain size?} \yt{It is ordered alphabetically be default. The domain size is to help calculate the domain size for the pair of interest from the reader side. One intuition is that the larger the domain size of a pair is, the less accuracy its corresponding metric would be. Maybe we don't have to show the numbers and simply sort the attributes by domain size to make the message simpler.}
In the title, "DepJac" corresponds to the jaccard distance between the set of dependent pairs and "CorAcc" corresponds to the accuracy of correlation levels in this dataset.
From this figure, we found that \algo{MST+}, \algo{MWEM-PGM+} and \algo{PrivBayes} all have similar correlation graphs with the one from ground truth, while \algo{Kamino+} has too many correlated attribute, \algo{FEM+} has some correlations under-estimated, \algo{RAP+} has some correlations over-estimated, and \algo{Independent+} and \algo{PATECTGAN} have all non-trivial correlations under-estimated.

Figure \ref{fig:pairdistribution} illustrates the pairwise distribution heatmap of a selected pair ("relationship", "marital-status") for one synthetic data generated by each algorithm given the private data "Adult" and $\epsilon=1.0$. In the title of each heatmap, "Cramer's V" indicates the correlation level of the selected pair in this dataset, and "L1 Score" measures the level of closeness by the L1 distance of this two-way marginal to the ground truth. A gray cell indicate there is no data. From this figure, we found that \algo{MST+}, \algo{MWEM-PGM+} and \algo{PrivBayes} all have similar distribution graphs with the one from ground truth, while \algo{Kamino+}, \algo{FEM+} and \algo{RAP+} capture some modes. \algo{Kamino+} also has a sparse distribution. \algo{Independent+} and \algo{PATECTGAN} all have independent distributions, but the shapes are different due to the difference on one-way marginals.\mh{should attribute values be ordered?} \yt{It is ordered by default alphabetically. Any preference for ordering?}


\subsection{Finding 2: Many Cannot Beat Baseline}

Depending on the metric for evaluating a synthetic data, some simple mechanisms could be viewed as baselines. For example, if the metric is measuring the similarity of the correlations between all the pairwise attributes, \algo{Independent+} is a baseline\mh{why is the name changed to `baseline' in the Fig. 3?  I think we should use the name independent everywhere.} \yt{Shall we keep its name independent in the figure, but we can say, it could be viewed as a baseline for some specific metrics when we analyze.} since it assumes all attributes are independent; if the metric is the accuracy of label classification, \algo{Independent+} is a baseline since training a reasonable classifier on an dataset with all the independent features and labels is similar to a majority classifier.

Our benchmark show that many mechanisms cannot beat baselines for correlation metrics and classification metrics. Figure \ref{fig:baseline}\mh{this should probably be two separate figures}  lists the raw score of "CorAcc" and "XGBoost" for datasets "Adult", "Shopping" and "Mushroom"\mh{why these datasets?}\yt{"Adult" is a sparsely-correlated dataset while "Mushroom" is a densely-correlated dataset. This could be a reason to choose these two datasets. In addition, "Mushroom" is a purely-categorical dataset, so it is fair to use this dataset to compare PrivTree with other mechanisms.} at $\epsilon=10$\mh{why epsilon=10?}\yt{I change epsilon to 1.0. A good reason for this choice is epsilon=1.0 is a reasonable bound for the total privacy loss (in convention?).} for all the mechanisms including the baseline. The score is taken as the average of scores from 5 runs. We use a diverging color scheme from blue to brown to indicate whether it is below or above the baseline. From this figure, we observe that many mechanisms have poorer performance than the baseline for some settings, except for \algo{MST+}, \algo{MWEM-PGM+} and \algo{PrivBayes}. Notice that for the dataset "Mushroom", the score "CorAcc" of the baseline is 0.13, which indicates that only 13\% of the attribute pairs in the original "Mushroom" are independent (with Cramer's V in [0, .1)), while this number is more than 50\% for other two datasets.

Fixing the dataset as "Adult", Figure \ref{fig:baseline} shows that \algo{Kamino+}, \algo{FEM+}, \algo{RAP+}, \algo{PATECTGAN}, \algo{DPCTGAN}, and \algo{RonGauss} all have better performance than the baseline in terms of classification accuracy, but all of them have worse performance than the baseline in terms of pairwise correlation. This is consistent from the observations in Figure \ref{fig:qualitative}, where these algorithms show they can capture the items that appear together frequently but the overall association or distribution might be less accurate.

\mh[inline]{add a conclusion.  briefly mention most important finding, but also include some discussion of limitations of our study}



\eat{
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{"figures/compact-correlation-Adult-epsilon-1.pdf"}
        \caption{The correlation heatmap of all pairwise categorical attributes for one synthetic data generated by each algorithm given the private data "Adult" and $\epsilon=1.0$.}
        \label{fig:correlation}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{"figures/compact-pair-distribution-Adult-relationship-marital-status-epsilon-1.pdf"}
        \caption{The pairwise distribution heatmap of the pair ("relationship", "marital-status") for one synthetic data generated by each algorithm given the private data "Adult" and $\epsilon=1.0$. }
        \label{fig:pairdistribution}
    \end{subfigure}
    \caption{The qualitative analysis of the synthetic data.}
    \label{fig:qualitative}
\end{figure}
}




\eat{
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.16\linewidth}
        \centering
        \adjustbox{trim={.0\width} {.0\height} {0.87\width} {.15\height},clip,width=\linewidth}%
        {\includegraphics[width=\linewidth]{"figures/Quantitative.png"}}
    \end{subfigure}
    \begin{subfigure}[t]{0.26\linewidth}
        \centering
        \adjustbox{trim={.14\width} {.0\height} {0.65\width} {.15\height},clip,width=\linewidth}%
        {\includegraphics[width=\linewidth]{"figures/Quantitative.png"}}
        \caption{Mix-Ind-L1 \label{fig:ind_l1}}
    \end{subfigure}
    %\begin{subfigure}[t]{0.1995\linewidth}
    %    \centering
    %    \adjustbox{trim={.35\width} {.0\height} {0.44\width} %{.15\height},clip,width=\linewidth}%
    %    {\includegraphics[width=\linewidth]{"figures/Quantitative.png"}%}
    %    \caption{Mix-Pair-L1 \label{fig:Mix-Pair-L1}}
    %\end{subfigure}
    \begin{subfigure}[t]{0.26\linewidth}
        \centering
        \adjustbox{trim={.57\width} {.0\height} {0.22\width} {.15\height},clip,width=\linewidth}%
        {\includegraphics[width=\linewidth]{"figures/Quantitative.png"}}
        \caption{CorAcc \label{fig:CorAcc}}
    \end{subfigure}
    \begin{subfigure}[t]{0.26\linewidth}
        \centering
        \adjustbox{trim={.79\width} {.0\height} {.0\width} {.15\height},clip,width=\linewidth}%
        {\includegraphics[width=\linewidth]{"figures/Quantitative.png"}}
        \caption{XGBoost \label{fig:XGBoost}}
    \end{subfigure}
    
    \caption{$\epsilon=1.0$.}
    \label{fig:my_label}
\end{figure}
}



==> experiments.tex <==
\section{Experimental Results}

\subsection{What tables or figures of experiments do we want to show and why?}

\begin{enumerate}
    \item Tables
    \begin{itemize}
        \item A universal table for "all experiment settings" $\times$ "all algorithms" $\times$ "all metrics". \mh{this seems impractical, won't it be too large?} \yt{Agree. Shall we just give a link to the universal table and remove the table itself from the paper? } \mh{sure}
        \item Sub-tables for each "metric group" as "all experiment settings" $\times$ "all algorithms"
        \item Sub-tables for each "dataset" as "all experiment settings of privacy budget" $\times$ "all algorithms" $\times$ "all metrics".
    \end{itemize}
    \item Figures
    \begin{itemize}
        \item A bar graph for each "dataset", for each "$\epsilon$", which is grouped by "metric" and hued by "algortihms".
    \end{itemize}
\end{enumerate}


\subsection{What main findings do we want to include or expect and why?}

Suppose we want to ask the following questions.
\begin{enumerate}
    \item What are the algorithms that are most scalable? 
    \item What are the algorithms that are most accurate in terms of distribution similarity of low-way marginals? 
    \item What are the algorithms that are most accurate in terms of distribution similarity on a graphical structure? 
    \item What are the algorithms that are most accurate in terms of discriminator-based distinguishability?
    \item What are the algorithms that are most useful for machine learning tasks?
    \item What are the algorithms that need least hyper-parameter tuning effort?
\end{enumerate}

\textbf{Overview}

\yt{add the main findings in summary.}

\yt{Bullet pioints corresponding to each finding.}

PrivTree vs Non-PrivTree

Runtime/Memory

\subsection{Runtime}

We begin by evaluating the runtime of each mechanism on each dataset and privacy parameter, and report whether it successfully completed without error under the 4 hour time limit.  The results are shown in \cref{fig:runtime}.  The plot is broken up into into groups of 3 columns, corresponding to three different privacy levels tested: $\epsilon = 0.1, 1.0, 10.0$.  Each cell of the heatmap corresponds to the time (in seconds) required to complete on the given dataset and privacy level, averaged across five trials.  Cells are colored white if the mechanism did not complete in all five trials for the given setting.  White cells are labeled either ``T'' or ``E'' to indicate the failure mode (timeout or error, respectively).

Not all mechanisms were able to complete successfully in every tested setting.  Some mechanisms simply timed out, while others encountered runtime errors.  The reason for failure differed by mechanism.  Kamino and the GAN-based methods mainly reached the runtime limit, while RAP often enountered the memory limit.  FEM reported an assertion error, and MWEM+PGM reported a NaN error for small privacy budgets.  The only mechanisms that ran successfully in every tested setting were MST and PrivBayes.  PrivBayes was quite fast, usually completing in under 10 seconds, and MST was also reasonably efficient, often running in less than 10 minutes.  Kamino and the GAN based methods were the most time consuming, requiring several hours on most datasets.  All of the implementations we use are ``research code'', so it is not surprising that some of them failed when run on new datasets which they were not originally evaluated on.  

It is interesting to note that FEM and the GAN-based methods required more runtime with larger $\epsilon$, as they run for more iterations.  It is also interesting to note that RAP failed to run by itself on some datasets (e.g., Adult), but RAP+PrivTree was able to run successfully on the same dataset.  This is likely due to the fact that PrivTree induces a coarser-grained discretization, that results smaller domain sizes, enabling RAP to be more efficient.

\begin{figure}
\includegraphics[]{figs/Runtime}
\caption{ \label{fig:runtime} Runtime. 
A. RonGauss
B. FEM
C. FEM+PrivTree
D. Kamino
E. Kamino+PrivTree
F. MST
G. MST+PrivTree
H. MWEM+PGM
I. MWEM+PGM+PrivTree
J. PrivBayes
K. RAP
L. RAP+PrivTree
M. DP-CTGAN
N. PATE-GAN }
\end{figure}



\subsection{1-way marginals (sanity check)}

We now evaluate each mechanism in terms of their accuracy on preserving 1-way marginals.  For this, we primarily look at two metrics: CSTest (for categorical attributes) and KSTest (for numerical attributes).  This is not a particularly interesting metric to look at: any reasonable mechanism should be able to easily preserve 1-way marginals well.  It thus serves as a useful sanity check for each mechanism.  

\cref{fig:cstest,fig:kstest} shows the performance of each mechanism on the CSTest and KSTest metrics, respectively.  MST, MWEM+PGM, and PrivBayes (and the PrivTree variants) all consistently score above $0.95$ on this metric across all datasets and privacy budgets considered.   Kamino and RAP (and the PrivTree variants) also perform reasonably well here, consistently scoring above $0.85$.   RonGauss, FEM, DP-CTGAN and PATE-GAN did not perform as well on this metric, in many cases scoring below $0.5$. \mh{FEM and DP-CTGAN seem to do ok on some datasets/epsilons -- e.g., FEM on Asia and Car has yellow squares in Fig. 2.}

Many mechanisms struggled to consistently score well on the KSTest.  In fact, the only mechanisms that consistently scored above $0.95$ on this metric were MST+PrivTree and MWEM+PGM+PrivTree.  With naive equi-width discretization, all mechanisms scored poorly, only reaching a score of $0.95$ or higher in a few cases.  This demonstrates the need to have a good data-dependent discretizer like PrivTree to score well on this metric.  

\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/CSTest}
\caption{ \label{fig:cstest} CSTest \mh{it's confusing that which cells are white varies from plot to plot}}
\end{figure}
\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/KSTest}
\caption{ \label{fig:kstest} KSTest}
\end{figure}

\subsection{2-way Marginals}

We now turn our attention to metrics that capture how well the synthetic data preserves 2-way marginals.  For that, we look at the DiscreteKLDivergence (for categorical attributes) and ContinuousKLDivergence (for numeric attributes) \footnote{SDGym does not have any 2-way marginal metrics that mix and match categorical and numerical attributes.}.  Preserving correlations in the underlying data is one of the main challenges synthetic data generators try to solve, and hence these metrics effectively capture general-purpose fitness-of-use for the synthetic data. 

\cref{fig:discretekl,fig:continuouskl} shows the performance of each mechanism on the DiscreteKLDivergence and ContinuousKLDivergence metrics, respectively.  Again, MST, MWEM+PGM, and PrivBayes (and the PrivTree variants) consistently do well on the DiscreteKLDivergence metric, across all datasets and privacy levels.  These mechanisms all score above $0.9$ when $\epsilon \geq 1$ for all datasets except Intrusion and Mushroom.  For those datasets, these mechanisms still score significantly higher than the alternatives. 

We observe similar behavior for ContinuousKLDivergence.  Somewhat surprisingly, PrivTree does not seem to help as much on this metric, and the naive equi-width discretization performs quite well here, especially with higher privacy budgets. 

\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/DiscreteKLDivergence}
\caption{ \label{fig:discretekl} DiscreteKLDivergence }
\end{figure}
\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/ContinuousKLDivergence}
\caption{ \label{fig:continuouskl} ContinuousKLDivergence }
\end{figure}

\subsection{Machine Learning Efficacy}

Next, we look at machine learning efficacy metrics.  That is, how well do machine learning models trained on synthetic data perform when evaluating on real data?  We show results for one popular machine learning algorithm, XGBoost in \cref{fig:xgboost}.  We include results on other machine learning algorithms in the appendix.

For this metric, none of the mechanisms were able to score above $0.9$ consistently.   This is not surprising, as even the non-private baseline does not score that high.  MWEM+PGM generally offers the best performance when it runs.  MST, PrivBayes, and RAP also achieve comparable scores (within $0.05$ of MWEM+PGM).  Other mechanisms are not competitive on this metric.

\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/MulticlassXGBoost.pdf}
\caption{\label{fig:xgboost} XGBoost}
\end{figure}
%\includegraphics[]{figs/MulticlassLogisticRegression.pdf}

\subsection{Discriminator-based Distinguishability}

Finally, we look at discriminator based distinguisiability metric --- specifically, the LogisticDetection metric.  As shown in \cref{fig:detection}, MST+PrivTree consistently achieves better scores than every other mechanism on this metric.  On some datasets (like Bank), the PrivTree variant is significantly better than the base mechanism.  This mechanism did not peform as well at $\epsilon=0.1$, but was still better than the alternatives in these cases. 

\begin{figure}[H]
\includegraphics[width=\textwidth]{figs/LogisticDetection.pdf}
\caption{\label{fig:detection} LogisticDetection }
\end{figure}

\subsection{Findings}

TODO: More descriptive headings

\begin{enumerate}
\item Many mechanisms failed to run successfully for all five trials on some datasets/settings (4 hour for one trial), either due to runtime errors, or time/memory limits. The reasons for failure differ by mechanism. The only methods that ran successfully on every tested dataset/epsilon were MST and PrivBayes.  GAN-based methods and Kamino were among the most expensive, often requiring hours and exceeding the time limit.  Runtime of FEM increased with epsilon.  PrivBayes consistently finished in under 10 seconds.  MST consistently finished in under 10 minutes.
\item Many methods failed to preserve 1-way marginals well (CSTest) \yt{See if KSTest failes as well)}. The only mechanisms that did well here are Kamino, MST, MWEM+PGM, PrivBayes, and to a lesser extent RAP. RonGauss, FEM, and the GAN-based methods did not consistently score well on this metric.  \mh{I think this finding is a little overly negative.  Of the 9 methods, 4 do well (Kamino, MST, MWEM+PGM, PrivBayes); 3 do well sometimes (RAP, FEM, DP-CTGAN) and 2 do poorly all the time (RonGauss, PATE-GAN).}
\item Using a PrivTree discretizer consistenly improves discretization.\mh{this doesn't seem entirely true given that the pareto frontier results.} All base mechanisms struggle on continuous columns (KSTest). Incorporating PrivTree discretizers improves performance.
 
\item \yt{Announce the winner} Pareto frontier includes MST, MWEM+PGM, PrivBayes, and Kamino, plus PrivTree variants.  MST a good default choice.  When PrivBayes wins, epsilon is high.
\item Metric-wise findings:
\begin{enumerate}
    \item MST and PrivBayes do a good job of preserving 2-way marginals (DiscreteKLDivergence, ContinuousKLDivergence). MWEM+PGM, Kamino, and RAP do a fairly good job here as well.
    \item MST+PrivTree and MWEM+PGM+PrivTree consistently did the best on the Logistic Detection metric. PrivTree discretization was key here.
    \item MWEM+PGM generally performed the best on the ML efficacy metrics.
    \end{enumerate}
\end{enumerate}
\item Feasibility in runtime?

\ry{add quantifiable measure to compare methods}

\ry{3 colors for plots}

\ry{giving algorithm more epsilon does not improve their performance enough}

\ry{possible critique: are GAN methods using best analysis?  Probably OK.}

\ry{emphasize algorithmic perspective compared to specific implementations.  Marginal based > GAN based (in intro).}

==> mechanisms.tex <==
\section{Mechanisms}

\ry{I think one stage inclusion criteria is fine.  Gretel seems to be the only thing excluded in step 2, we can just treat that as a special case} 

We consider a two-stage benchmark that includes the algorithms using the inclusion criteria for each stage. See Section \ref{sec:motivation-two-stage} for more details. 

\subsection{Stage 1 Inclusion Criteria}
We consider benchmarking the algorithms satisfying the following criteria:

\begin{enumerate}
    \item \textbf{End-to-End DP}: It is claimed to be end-to-end differential private algorithm that generates synthetic data in tabular form.
    %\yt{For some algorithms, we found privacy breaches in the implementations, e.g. DPCTGAN from QUAIL. How should we include them?}\am{If you want o include DPCTGAN, maybe you can say "claimed to be end to end DP"} \yt{end-to-end to remove?}
    \item \textbf{Tabular Data}: It supports tabular data that could have numerical columns, categorical columns, or both. The original paper should have experiments on tabular data.
    %\item It should have been published for at least one year. \yt{Do we want to include this criterion?} \am{What does this mean? Published in 2020 or before? What gets eliminated by this criterion? Kamino?}
    \item \textbf{Selected Field}: It is published in a top conference or included in a well known library. For conferences, we consider SIGMOD, VLDB, CCS, NeurIPS, ICML, PETS and JPC . For libraries, we consider SmartNoise and Gretel. \yt{We could say, we just include them but it doesn't mean confs outside is not top.}
    %\mh{... and Gretel?  it appears to be included in stage 1.}
    %\yt{Some algorithms are published in arxiv or not even published. How should we include them?}\am{One idea is to add a disjunction: Top conference or included in a well known library like SmartNoise?}
    \item \textbf{Open Source}: It has open-source codes accessible to the public such that it could be either found from GitHub or its link is included in the paper. \yt{We implement MST and MWEMPGM inside Tumult library. How should we include it into the criteria?}
    \item \textbf{No Extra Data}: It should be able to run with only the sensitive data and its data schema.
\end{enumerate}

Table \ref{tab:inclusion} lists the algorithms we included in this benchmark:
%\yt{We also have variants of MST, MWEMPGM and PrivBayes with different column discretizers. They should be included in the table as well, but I'm not sure how to represent them.}
\begin{table}[h!]
    \centering
    \begin{tabular}{|p{2.5cm}|p{4cm}|p{3.5cm}|p{3cm}|}
    \hline
        \textbf{Algorithm} & \textbf{Published In} & \textbf{Implementation} & \textbf{Pre/Post-Processing}  \\ \hline
        MST & JPC? & PGM(github) & discretization\\ \hline
        MWEMPGM & ICML \cite{mckenna2019graphical} &  PGM(github) \tablefootnote{needs modification in the github} & discretization\\ \hline
        PrivBayes & SIGMOD \cite{DBLP:conf/sigmod/ZhangCPSX14}, TODS \cite{zhang2017privbayes} & SDGym & discretization ? \\ \hline
        DPGAN\tablefootnote{\yt{not yet benchmarked} }  & CoRR \cite{DBLP:journals/corr/abs-1802-06739} & SmartNoise & embedding\\ \hline
        DPCTGAN\tablefootnote{privacy breach issue} & CoRR \cite{rosenblatt2020differentially} & SmartNoise & N/A \\ \hline
        PATEGAN & ICLR \cite{DBLP:conf/iclr/JordonYS19a} & SmartNoise & embedding \\ \hline
        PATECTGAN\tablefootnote{\yt{not yet benchmarked} } & ICLR \cite{rosenblatt2020differentially} & SmartNoise & N/A \\ \hline
        Kamino & PVLDB \cite{DBLP:journals/pvldb/GeMHI21} & Ge  & discretization \\ \hline
        FEM & ICML \cite{DBLP:conf/icml/VietriTBSW20} & Vietri & discretization \\ \hline
        RAP & ICML \cite{DBLP:conf/icml/AydoreBKKM0S21} & Amazon &  discretization \\ \hline
        RON-GAUSS & PETS \cite{DBLP:journals/popets/ChanyaswadLM19} & BorealisAI &  embedding \\ \hline
        GretelRNN\tablefootnote{Gretel & removed in Stage 2 } & blog & Gretel & N/A \\ \hline
    \end{tabular}
    \caption{Algorithms included 
    %\mh{we need more algorithms!}
    }
    \label{tab:inclusion}
\end{table}

By default, we use one-hot encoding for learning the embedding. For discretization, we have two strategies: 100 equal-width bins or learning the bining using PrivTree by paying a small portion of budget. \yt{Shall we study the choice of discretization in stage 1 or just compare all the variants in stage 2?}

\yt{Add the Quantile discretization? Maybe just say we tried and compared for a limited setting.}

\eat{
Table \ref{tab:to_include} is the algorithms that we will consider or further include in this benchmark.
\begin{table}[h!]
    \centering
    \begin{tabular}{|p{2.5cm}|p{3cm}|p{3.5cm}|p{6cm}|}
    \hline
        \textbf{Algorithm} & \textbf{Published In} & \textbf{Open-source Link} & \textbf{Note}  \\ \hline
        %DP-MERF & AISTATS \cite{DBLP:conf/aistats/HarderAP21} & Github (ParkLabML) & 1) It has codes 2) It supports tabular data \\ \hline
        %DP-CGAN & CVPR(W) \cite{DBLP:conf/cvpr/Torkzadehmahani19} & Github &  \\ \hline
        %GS-WGAN & NeurIPS \cite{neurips20chen} & Github & \\ \hline
    \end{tabular}
    \caption{Algorithms to consider / include \mh{please add comments on why or why not include}}
    \label{tab:to_include}
\end{table}
}

Table \ref{tab:exclusion} is the algorithms that we considered but not included in this benchmark or we tested but there were some issues. \yt{We might need to have a section for discussing about these algorithms.}
\begin{table}[H]
    \centering
    \begin{tabular}{|p{4.5cm}|p{3cm}|p{4.5cm}|}
    \hline
        Algorithm & Published In & Violated Inclusion Criteria \\ \hline
        PrivateIMLE  \tablefootnote{The original paper is not differentially private. BorealisAI adapted the original algorithm and claimed it follows differential privacy.} & CoRR \cite{DBLP:journals/corr/abs-1809-09087} & Selected Field  \\ \hline
        DPSynthesizer / DPCopula  & PVLDB \cite{DBLP:journals/pvldb/LiXZJ14} & Open Source  \\ \hline
        DPSyn & CoRR \cite{DBLP:journals/corr/abs-2106-12949} & Open Source \\ \hline
        PrivSyn & CoRR \cite{DBLP:journals/corr/abs-2012-15128} & Open Source  \\ \hline
        PMWPub & ICML \cite{DBLP:conf/icml/LiuV0UW21} & No Extra Data  \\ \hline
        PEP / GEM / GEMPUB  & CoRR \cite{DBLP:journals/corr/abs-2106-07153} & Selected Field  \\ \hline
        pMSE & PSD \cite{DBLP:conf/psd/SnokeS18} & Open Source  \\ \hline
        DP-MERF \tablefootnote{It supports tabular data and is implemented by ParkLabML} & AISTATS \cite{DBLP:conf/aistats/HarderAP21} & Selected Field   \\ \hline
        DP-CGAN & CVPR(W) \cite{DBLP:conf/cvpr/Torkzadehmahani19} & Selected Field  \\ \hline
        GS-WGAN & NeurIPS \cite{neurips20chen} & Tabular Data  \\ \hline
        
    \end{tabular}
    \caption{Algorithms considered but not included or found some issues.}
    \label{tab:exclusion}
\end{table}

\subsection{Stage 2 Inclusion Criteria}

\yt{Maybe we can move this to the stage 1 as a minor criteria for rejecting GretelRNN}.

GretelRNN uses rejection sampling for the sampling step but the rejection rate is high and it could not generate a single record in 15 minutes after it finishes the model learning of the "asia" dataset with the default parameters. The reported epsilon is also as high as 4205431.

Table \ref{tab:stage2-exclusion} shows the algorithms included in the stage 1 but excluded for the stage 2. 

\begin{table}[H]
    \centering
    \begin{tabular}{|p{2.5cm}|p{3cm}|p{3.5cm}|p{6cm}|}
    \hline
        Algorithm & Published In & Open-source Link  & Note \\ \hline
        GretelRNN & blog & Github(Gretel) & 1) no data generated 2) privacy breach \\ \hline
        %DPGAN  & CoRR \cite{DBLP:journals/corr/abs-1802-06739} & Github(SmartNoise) & \yt{check Quail to see if it is much worse than other algorithms} \\ \hline
        
    \end{tabular}
    \caption{Algorithms excluded in Stage 2.}
    \label{tab:stage2-exclusion}
\end{table}

==> outline.tex <==
\section{Inclusion Criteria}\label{sec:inclusion}

We consider a two-stage benchmark that includes the algorithms using the inclusion criteria for each stage. See Section \ref{sec:motivation-two-stage} for more details. 

\subsection{Stage 1 Inclusion Criteria}
We consider benchmarking the algorithms satisfying the following criteria:

\begin{enumerate}
    \item \textbf{End-to-End DP}: It is claimed to be end-to-end differential private algorithm that generates synthetic data. 
    %\yt{For some algorithms, we found privacy breaches in the implementations, e.g. DPCTGAN from QUAIL. How should we include them?}\am{If you want o include DPCTGAN, maybe you can say "claimed to be end to end DP"} \yt{end-to-end to remove?}
    \item \textbf{Tabular Data}: It supports tabular data that could have numerical columns, categorical columns, or both. The original paper should have experiments on tabular data.
    %\item It should have been published for at least one year. \yt{Do we want to include this criterion?} \am{What does this mean? Published in 2020 or before? What gets eliminated by this criterion? Kamino?}
    \item \textbf{Selected Field}: It is published in a top conference or included in a well known library. For conferences, we consider SIGMOD, VLDB, CCS, NeurIPS, ICML, PETS, JPC and CoRR \mh{CoRR is not a top conference!}. For libraries, we consider SmartNoise and Gretel. 
    %\mh{... and Gretel?  it appears to be included in stage 1.}
    %\yt{Some algorithms are published in arxiv or not even published. How should we include them?}\am{One idea is to add a disjunction: Top conference or included in a well known library like SmartNoise?}
    \item \textbf{Open Source}: It has open-source codes accessible to the public such that it could be either found from GitHub or its link is included in the paper. \yt{We implement MST and MWEMPGM inside Tumult library. How should we include it into the criteria?}
    \item \textbf{No Extra Data}: It should be able to run with only the sensitive data and its data schema.
\end{enumerate}

Table \ref{tab:inclusion} lists the algorithms we included in this benchmark:
%\yt{We also have variants of MST, MWEMPGM and PrivBayes with different column discretizers. They should be included in the table as well, but I'm not sure how to represent them.}
\begin{table}[h!]
    \centering
    \begin{tabular}{|p{2.5cm}|p{4cm}|p{3.5cm}|p{3cm}|}
    \hline
        \textbf{Algorithm} & \textbf{Published In} & \textbf{Implementation} & \textbf{Pre/Post-Processing}  \\ \hline
        MST & JPC? & PGM(github) & discretization\\ \hline
        MWEMPGM & ICML \cite{mckenna2019graphical} &  PGM(github) \tablefootnote{needs modification in the github} & discretization\\ \hline
        PrivBayes & SIGMOD \cite{DBLP:conf/sigmod/ZhangCPSX14}, TODS \cite{zhang2017privbayes} & SDGym & discretization \\ \hline
        DPGAN\tablefootnote{\yt{not yet benchmarked} }  & CoRR \cite{DBLP:journals/corr/abs-1802-06739} & SmartNoise & embedding\\ \hline
        DPCTGAN\tablefootnote{privacy breach issue} & CoRR \cite{rosenblatt2020differentially} & SmartNoise & N/A \\ \hline
        PATEGAN & ICLR \cite{DBLP:conf/iclr/JordonYS19a} & SmartNoise & embedding \\ \hline
        PATECTGAN\tablefootnote{\yt{not yet benchmarked} } & ICLR \cite{rosenblatt2020differentially} & SmartNoise & N/A \\ \hline
        Kamino & PVLDB \cite{DBLP:journals/pvldb/GeMHI21} & Ge  & discretization \\ \hline
        FEM & ICML \cite{DBLP:conf/icml/VietriTBSW20} & Vietri & discretization \\ \hline
        RAP & ICML \cite{DBLP:conf/icml/AydoreBKKM0S21} & Amazon &  discretization \\ \hline
        RON-GAUSS & PETS \cite{DBLP:journals/popets/ChanyaswadLM19} & BorealisAI &  embedding \\ \hline
        GretelRNN\tablefootnote{Gretel & removed in Stage 2 } & blog & Gretel & N/A \\ \hline
    \end{tabular}
    \caption{Algorithms included 
    %\mh{we need more algorithms!}
    }
    \label{tab:inclusion}
\end{table}

By default, we use one-hot encoding for learning the embedding. For discretization, we have two strategies: 100 equal-width bins or learning the bining using PrivTree by paying a small portion of budget. \yt{Shall we study the choice of discretization in stage 1 or just compare all the variants in stage 2?}

\eat{
Table \ref{tab:to_include} is the algorithms that we will consider or further include in this benchmark.
\begin{table}[h!]
    \centering
    \begin{tabular}{|p{2.5cm}|p{3cm}|p{3.5cm}|p{6cm}|}
    \hline
        \textbf{Algorithm} & \textbf{Published In} & \textbf{Open-source Link} & \textbf{Note}  \\ \hline
        %DP-MERF & AISTATS \cite{DBLP:conf/aistats/HarderAP21} & Github (ParkLabML) & 1) It has codes 2) It supports tabular data \\ \hline
        %DP-CGAN & CVPR(W) \cite{DBLP:conf/cvpr/Torkzadehmahani19} & Github &  \\ \hline
        %GS-WGAN & NeurIPS \cite{neurips20chen} & Github & \\ \hline
    \end{tabular}
    \caption{Algorithms to consider / include \mh{please add comments on why or why not include}}
    \label{tab:to_include}
\end{table}
}

Table \ref{tab:exclusion} is the algorithms that we considered but not included in this benchmark or we tested but there were some issues. \yt{We might need to have a section for discussing about these algorithms.}
\begin{table}[H]
    \centering
    \begin{tabular}{|p{4.5cm}|p{3cm}|p{4.5cm}|}
    \hline
        Algorithm & Published In & Violated Inclusion Criteria \\ \hline
        PrivateIMLE  \tablefootnote{The original paper is not differentially private. BorealisAI adapted the original algorithm and claimed it follows differential privacy.} & CoRR \cite{DBLP:journals/corr/abs-1809-09087} & Selected Field  \\ \hline
        DPSynthesizer / DPCopula  & PVLDB \cite{DBLP:journals/pvldb/LiXZJ14} & Open Source  \\ \hline
        DPSyn & CoRR \cite{DBLP:journals/corr/abs-2106-12949} & Open Source \\ \hline
        PrivSyn & CoRR \cite{DBLP:journals/corr/abs-2012-15128} & Open Source  \\ \hline
        PMWPub & ICML \cite{DBLP:conf/icml/LiuV0UW21} & No Extra Data  \\ \hline
        PEP / GEM / GEMPUB  & CoRR \cite{DBLP:journals/corr/abs-2106-07153} & Selected Field  \\ \hline
        pMSE & PSD \cite{DBLP:conf/psd/SnokeS18} & Open Source  \\ \hline
        DP-MERF \tablefootnote{It supports tabular data and is implemented by ParkLabML} & AISTATS \cite{DBLP:conf/aistats/HarderAP21} & Selected Field   \\ \hline
        DP-CGAN & CVPR(W) \cite{DBLP:conf/cvpr/Torkzadehmahani19} & Selected Field  \\ \hline
        GS-WGAN & NeurIPS \cite{neurips20chen} & Tabular Data  \\ \hline
        
    \end{tabular}
    \caption{Algorithms considered but not included or found some issues.}
    \label{tab:exclusion}
\end{table}

\subsection{Stage 2 Inclusion Criteria}

\yt{Maybe we can move this to the stage 1 as a minor criteria for rejecting GretelRNN}.

GretelRNN uses rejection sampling for the sampling step but the rejection rate is high and it could not generate a single record in 15 minutes after it finishes the model learning of the "asia" dataset with the default parameters. The reported epsilon is also as high as 4205431.

Table \ref{tab:stage2-exclusion} shows the algorithms included in the stage 1 but excluded for the stage 2. 

\begin{table}[H]
    \centering
    \begin{tabular}{|p{2.5cm}|p{3cm}|p{3.5cm}|p{6cm}|}
    \hline
        Algorithm & Published In & Open-source Link  & Note \\ \hline
        GretelRNN & blog & Github(Gretel) & 1) no data generated 2) privacy breach \\ \hline
        %DPGAN  & CoRR \cite{DBLP:journals/corr/abs-1802-06739} & Github(SmartNoise) & \yt{check Quail to see if it is much worse than other algorithms} \\ \hline
        
    \end{tabular}
    \caption{Algorithms excluded in Stage 2.}
    \label{tab:stage2-exclusion}
\end{table}



\section{Benchmark Design}

\ry{Maybe state that we are building on top of SDGym, so we can cite them and not have to justify benchmark setup as much.}


\subsection{The motivation of two stage benchmark}\label{sec:motivation-two-stage}
A tabular data could include both categorical and numerical columns, but not all algorithms can handle mixed type data naturally. To compare these algorithms, we propose several options
\begin{enumerate}
    \item Option 1: We only compare algorithms on datasets that algorithms support.
    \item Option 2: Add a data-independent pre/post-processor to those algorithms that do not support one of the types.  (No budget required for these data-ind pre-processors.) \ry{This is what we have already done, so I think we have to go with Option 2.}
    \item Option 3: Pre-process datasets: this lets algorithms run un-modified, but prevents comparison of different algorithm types.  This is essentially a variant of 1 (we're just adding more datasets).
    \item Option 4: Do a small study on transformers and adopt a `best of' model (which will likely be data-dedependent).  Apply this pre/post-processor to those algorithms that do not support one of the types. The pre-processor may consume some privacy-budget.
\end{enumerate}

To apply option 4, we consider a two-stage benchmark. In the first stage, we include algorithms that satisfy the Stage 1 inclusion criteria (see Section \ref{sec:inclusion}) and we launch an initial benchmark with data-independent pre/pro-processors to filter the algorithms according to Stage 2 inclusion criteria. Then we study the pre/post-processor for the algorithms as described by Option 4. In the second stage, we launch a full-fledged benchmark for the candidates selected from the previous stage. All candidates are equipped with the pre/post-processors studied in the fist stage.




\subsection{What evaluation metrics do we want to include and why?}

\begin{enumerate}
    \item Synthetic Data Quality \ry{I think we should consider CSTest, KSTest, DiscreteKL, ContinuousKL, LogisticDetection, and MulticlassXGBoost.  All of these except the last are already implemented in SDGym so I think it's well-justified to use existing metrics.  Maybe we should even switch MulticlassXGBoost with MulticlassLogisticRegression so that we can say all metrics are in SDGym.  I think there are some really nice visualizations involving 2-way marginals we should incorporate somewhere as well.}
    \begin{itemize}
        \item Distribution Similarity of low-way Marginals
        \begin{itemize}
            \item average/max one-way (nominal) marginal CS-Test
            \item average/max one-way (ordinal) marginal KS-Test
            \item average/max two-way (nominal) marginal KL Divergence
            \item average/max two-way (ordinal) marginal KL Divergence
        \end{itemize}
        \item Distribution Similarity on a Graphical Structure
        \begin{itemize}
            \item Bayesian Network
            \begin{itemize}
                \item Strategy
                \begin{itemize}
                    \item Option 1: Train BN from Real and sample Syn.
                    \item Option 2: Train BN from Syn and sample Real.
                \end{itemize}
                \item Likelihood
                \begin{itemize}
                    \item Option 1: Multinomial distribution with fixed n.
                    \item Option 2: Average likelihood with non-fixed n.
                \end{itemize}
            \end{itemize}
        \end{itemize}
        \item Discriminator-based Distinguishability
        \begin{itemize}
            \item p-MSE \cite{DBLP:conf/psd/SnokeS18} \am{Is this the Joshua Snoke metric?} \yt{Yes}
        \end{itemize}
        \item Machine Learning Utility (Train Real/Synthetic, Test Real)  \mh{do we really need to train all of these models?} \yt{We can run and just keep the ones we want.}
        \begin{itemize}
            \item XGBoost
            \item LightGBM
            \item CatBoost
            \item Decision Tree
            \item AdaBoost
            \item Logistic Regression
            \item Bagging
            \item Random Forest
        \end{itemize}
        \item More ...
        \begin{itemize}
            \item More ...
        \end{itemize}
    \end{itemize}
    \item Scalability
    \begin{itemize}
        \item Runtime
        \item Memory
    \end{itemize}
    \item{Hardness of Tuning Hyperparameters}
    \begin{itemize}
        \item number of hyperparameters
        \item sensitivity of hyperparameters \mh{how is this measured?} \yt{We can measure how the metric values change if we change hyperparameters, which could be done in Stage 1. However, I think we can just leave this as a future work. }
        \item whether default hyperparameters exist
    \end{itemize}
\end{enumerate}

\subsection{What experiment settings do we want to have and why?}

\begin{enumerate}
    \item Privacy Budget
    \begin{itemize}
        \item Fix $\delta$ as $10^{-7}$ (smaller than 1/n for all the cases)
        \item Vary $\epsilon$ within $[0.1, 1.0, 10.0]$
    \end{itemize}
    \item Datasets
    \begin{itemize}
        \item Consider datasets of different dimensions, data size, column types.
        \item "adult", 9 cat, 6 num, 1 label, 32561 records
        \item "asia", 8 cat, 0 num, 0 label, 20000 records
        \item "census", 29 cat, 12 num, 1 label, 299285 records
        \item "covtype", 1 cat, 54 num, 1 label, 581012 records
        \item "EchoNASDAQ", 3 cat, 4 num, 0 label, 51980 records
        \item "intrusion", 4 cat, 37 num, 1 label, 494021 records
        \item "QuailAdult",  \mh{what's up with the `Quail' datasets?  how differ from the original dataset on which they are based?}
        \item "QuailBank",
        \item "QuailCar",
        \item "QuailMushroom",
        \item "QuailShopping",
        \item "GretelScooter",
        
    \end{itemize}
\end{enumerate}

\subsection{What tables or figures of experiments do we want to show and why?}

\begin{enumerate}
    \item Tables
    \begin{itemize}
        \item A universal table for "all experiment settings" $\times$ "all algorithms" $\times$ "all metrics". \mh{this seems impractical, won't it be too large?} \yt{Agree. Shall we just give a link to the universal table and remove the table itself from the paper? } \mh{sure}
        \item Sub-tables for each "metric group" as "all experiment settings" $\times$ "all algorithms"
        \item Sub-tables for each "dataset" as "all experiment settings of privacy budget" $\times$ "all algorithms" $\times$ "all metrics".
    \end{itemize}
    \item Figures
    \begin{itemize}
        \item A bar graph for each "dataset", for each "$\epsilon$", which is grouped by "metric" and hued by "algortihms".
    \end{itemize}
\end{enumerate}


\subsection{What main findings do we want to include or expect and why?}

Suppose we want to ask the following questions.
\begin{enumerate}
    \item What are the algorithms that are most scalable? 
    \item What are the algorithms that are most accurate in terms of distribution similarity of low-way marginals? 
    \item What are the algorithms that are most accurate in terms of distribution similarity on a graphical structure? 
    \item What are the algorithms that are most accurate in terms of discriminator-based distinguishability?
    \item What are the algorithms that are most useful for machine learning tasks?
    \item What are the algorithms that need least hyper-parameter tuning effort?
\end{enumerate}

\section{Related Benchmark/Comparison/Metric Papers}
In this section we review the existing benchmark papers, the comparative studies about differentially private synthetic data generation, or the work about its related metrics.

\begin{enumerate}
    \item {[Benchmark]} Smartnoise benchmark (DPSDGYM) along with QUAIL. \cite{rosenblatt2020differentially}
    \item {[Benchmark]} Benchmark principles \cite{DBLP:conf/sigmod/HayMMCZ16}.
    \item {[Benchmark]} Benchmark GAN variants under DP \cite{DBLP:journals/pvldb/FanLLCSD20}.
    \item {[Comparison]} Comparative Study of Differentially Private Synthetic Data Algorithms from the NIST PSCR Differential Privacy Synthetic Data Challenge \cite{bowen2019comparative}.
    \item {[Comparison]} This comparative study paper focuses more on old DPSDG papers ($\leq 2016$) \cite{bowen2020comparative}.
    \item {[Metric]} This working paper discusses the usefulness of synthetic data. \cite{DBLP:journals/corr/abs-2004-07740}
    \item {[Metric]} ML privacy meter (with codes) \cite{DBLP:journals/corr/abs-2007-09339}.
    \item {[Metric]} Evaluating DP ML \cite{DBLP:conf/uss/Jayaraman019}.
    \item {[Metric]} Sinkhorn distance between synthetic and ground-truth data \cite{DBLP:conf/aistats/GenevayPC18}.
    \item {[Metric]} The performance of ML model on the synthetic train/test should be similar to the case when given real train/test \cite{DBLP:journals/corr/abs-1806-11345}.
\end{enumerate}

\section{Algorithm Issues}

\subsection{General Issues}

\begin{enumerate}
    \item \textbf{Heavy requirements of computational resources.} Some algorithms are memory-heavy; e.g., Kamino consumes more than 5GB for the adult dataset.
    \item \textbf{Over-consume the total privacy budget.} Algorithms like SmartNoise DP-CTGAN don't split the budget in advance. It has a fixed noise scale for each round and use the composition theorem to calculate the consumption after each round to decide whether it should stop. The issue is, when it stops, it has already over-consume the privacy budget. 
    \item \textbf{No interface for setting the total privacy budget.} Algorithms like Kamino doesn't specify the total privacy budget it will consume. Instead, it only provides the interface to set the noise scale and the number of iterations. In the paper they described an algorithm to search the parameters that can make the main algorithm satisfy specified ($\epsilon, \delta$)-DP, but this algorithm is missing in the github implementation.  \mh{should we make this a criterion?} \yt{Yeah it could be. Under this criterion Kamino would be ruled out, but I added a routine to choose privacy parameters according to the total privacy budget, so right now Kamino is fine.}
    \item \textbf{Problematic implementation of "amplification by sub-sampling".} It is common in DP-SDG based algorithms to use sub-sampling to amplify the privacy. However, in the implementation of Gretel-RNN, instead of sampling with replacement, a random permutation of the data is applied and it becomes sampling without replacement. How it affects the privacy amplification? In the implementation of DP-CTGAN, it samples data conditionally. How should the "amplification by sub-sampling" rule be applied here? How should the privacy cost be analyzed? Sampling a database with sampling probability $q$ for each tuple is different from sampling $q$ fraction tuples from the database. However, in the implementation of Kamino, only data size and batch size are set as parameters, and each time of SGD a batch of the size "batch size" is sampled.
    \item \textbf{Active domain leaks information.} Some algorithms infer the full domain from the active domain, which could leak a lot of information if the active domain is sparse compared to the full domain. One example is the implementation of Kamino \yt{double check}, DPCTGAN, PATECTGAN.  \ry{Every mechanism we study looks at the active domain, not necessarily because of the mechanism, but because of the way SDGym is setup (datasets are not equipped with domain information).  Mechanisms whose internal implementation looks at the active domain are particularly problematic though.}
    
\end{enumerate}

\subsection{Bounded DP vs. Unbounded DP}

The interface for the total privacy budget.

Handling the comparison between unbounded and bounded DP. 

Proposed method: 

1) use the epsilons with the power of 2 to allow comparisons. 

2) use a small portion to estimate the total.

3) (choose it) just mark it

==> related.tex <==
\section{Related Work}

In this section we review the existing benchmark papers, the comparative studies about differentially private synthetic data generation, or the work about its related metrics.

\begin{enumerate}
    \item {[Benchmark]} Smartnoise benchmark (DPSDGYM) along with QUAIL. \cite{rosenblatt2020differentially}
    \item {[Benchmark]} Benchmark principles \cite{DBLP:conf/sigmod/HayMMCZ16}.
    \item {[Benchmark]} Benchmark GAN variants under DP \cite{DBLP:journals/pvldb/FanLLCSD20}.
    \item {[Comparison]} Comparative Study of Differentially Private Synthetic Data Algorithms from the NIST PSCR Differential Privacy Synthetic Data Challenge \cite{bowen2019comparative}.
    \item {[Comparison]} This comparative study paper focuses more on old DPSDG papers ($\leq 2016$) \cite{bowen2020comparative}.
    \item {[Metric]} This working paper discusses the usefulness of synthetic data. \cite{DBLP:journals/corr/abs-2004-07740}
    \item {[Metric]} ML privacy meter (with codes) \cite{DBLP:journals/corr/abs-2007-09339}.
    \item {[Metric]} Evaluating DP ML \cite{DBLP:conf/uss/Jayaraman019}.
    \item {[Metric]} Sinkhorn distance between synthetic and ground-truth data \cite{DBLP:conf/aistats/GenevayPC18}.
    \item {[Metric]} The performance of ML model on the synthetic train/test should be similar to the case when given real train/test \cite{DBLP:journals/corr/abs-1806-11345}.
\end{enumerate}
